AI Empowered Resource Management for Future Wireless Networks

Resource management plays a pivotal role in wireless networks, which, unfortunately, leads to challenging NP-hard problems. Artificial Intelligence (AI), especially deep learning techniques, has recently emerged as a disruptive technology to solve such challenging problems in a real-time manner. However, although promising results have been reported, practical design guidelines and performance guarantees of AI-based approaches are still missing. In this paper, we endeavor to address two fundamental questions: 1) What are the main advantages of AI-based methods compared with classical techniques; and 2) Which neural network should we choose for a given resource management task. For the first question, four advantages are identified and discussed. For the second question, \emph{optimality gap}, i.e., the gap to the optimal performance, is proposed as a measure for selecting model architectures, as well as, for enabling a theoretical comparison between different AI-based approaches. Specifically, for $K$-user interference management problem, we theoretically show that graph neural networks (GNNs) are superior to multi-layer perceptrons (MLPs), and the performance gap between these two methods grows with $\sqrt{K}$.

==> AI Empowered Resource Management for Future Wireless Networks/deleted.tex <==
they suffer from loss mismatch and performs badly when the optimal solution is not unique. We first elaborate the loss mismatch issue by considering the following power control problem
\begin{equation}\label{eq:pow_contr}
\begin{aligned}
&\underset{\vct{p} \in \mathbb{R}^K}{\text{maximize}}
& & \sum_{k=1}^{K} \log_2 \left(1+ \frac{h_{kk}p_k}{\sum_{i\neq k}h_{ki}p_i+1} \right) \\
& \text{subject to}
& & 0 \leq p_k \leq 1, 
\end{aligned}
\end{equation}
with an extreme channel gain matrix 
\begin{align*}
    H = \begin{bmatrix}
        100 & 0 & \infty & \infty & \infty \\
        0 & 100 & \infty & \infty & \infty \\
        \infty & \infty & 1 & \infty & \infty \\
         \infty & \infty & \infty &100 & 0   \\
        \infty & \infty & \infty & 0 & 99.9
    \end{bmatrix}.
\end{align*}

The optimal solution is given by $\bm{p} = [1,1,0,0,0]$ with sum rate $13.287$. Like in \cite{sun2018learning}, we adopt MSE loss to learn the solution. If the neural network outputs $\bm{p} = [1,1,1,0,0]$, the MSE loss is $1$ but sum rate is $0$. If the neural network outputs $\bm{p} = [0,0,0,1,1]$, the MSE loss is $4$ while the sum rate is $13.286$. Although the example in \eqref{eq:pow_contr} is extreme, it shows that a low MSE loss does not necessarily result in a high sum rate.



\begin{proposition}
    Suppose the , and $g$ is $(M, \epsilon, \delta)$ learable with $\mathcal{A}$, then 
    \begin{align*}
        \mathcal{E}_{test} \leq \epsilon
    \end{align*}
\end{proposition}

Training neural networks is basically a parameter estimation task. Thus, for a better understanding of PAC-theory, we begin with a trivial example, i.e., estimating the mean of bounded random variables. 
\begin{example}
     Let $X_1, \cdots, X_M$ be bounded i.i.d. random variables in $[b, b + B]$ and $y_i = g(x_i) = \mathbb{E}(X_i)$. 
\end{example}

We begin with the famous Hoeffding’s inequality. 
\begin{theorem} (Theorem 2.2.6 in \cite{vershynin2018high}) 
    Let $X_1, \cdots, X_M$ be bounded i.i.d. random variables in $[b, b + B]$. Then for any $t >0$, then exists an absolute constant $C$, such that 
    \begin{align*}
        \mathbb{P} \left\{ \sum_{i=1}^M \frac{1}{M} (X_i - \mathbb{E} X_i) \geq t \right\}  \leq \exp\left( -\frac{2t^2}{MB^2} \right).
    \end{align*}
\end{theorem}
Then we rewrite it in the terminology of PAC-learnable. 

\begin{proposition} (A Example of Learnability)\label{pro:high}
    Let $x_i$ be bounded random variables, $y_i = g(x_i) = \mathbb{E}(x_i)$, then $g$ is $(M, B\sqrt{\frac{1}{2M} \log \delta}, \delta)$-learnable and 
    \begin{align*}
        \mathcal{E}_{\text{test}} \leq B\sqrt{\frac{1}{2M} \log \delta}.
    \end{align*}
\end{proposition}

From Proposition \ref{pro:high}, the optimality gap is a decreasing function of sample complexity $M$.

==> deleted.tex <==
they suffer from loss mismatch and performs badly when the optimal solution is not unique. We first elaborate the loss mismatch issue by considering the following power control problem
\begin{equation}\label{eq:pow_contr}
\begin{aligned}
&\underset{\vct{p} \in \mathbb{R}^K}{\text{maximize}}
& & \sum_{k=1}^{K} \log_2 \left(1+ \frac{h_{kk}p_k}{\sum_{i\neq k}h_{ki}p_i+1} \right) \\
& \text{subject to}
& & 0 \leq p_k \leq 1, 
\end{aligned}
\end{equation}
with an extreme channel gain matrix 
\begin{align*}
    H = \begin{bmatrix}
        100 & 0 & \infty & \infty & \infty \\
        0 & 100 & \infty & \infty & \infty \\
        \infty & \infty & 1 & \infty & \infty \\
         \infty & \infty & \infty &100 & 0   \\
        \infty & \infty & \infty & 0 & 99.9
    \end{bmatrix}.
\end{align*}

The optimal solution is given by $\bm{p} = [1,1,0,0,0]$ with sum rate $13.287$. Like in \cite{sun2018learning}, we adopt MSE loss to learn the solution. If the neural network outputs $\bm{p} = [1,1,1,0,0]$, the MSE loss is $1$ but sum rate is $0$. If the neural network outputs $\bm{p} = [0,0,0,1,1]$, the MSE loss is $4$ while the sum rate is $13.286$. Although the example in \eqref{eq:pow_contr} is extreme, it shows that a low MSE loss does not necessarily result in a high sum rate.



\begin{proposition}
    Suppose the , and $g$ is $(M, \epsilon, \delta)$ learable with $\mathcal{A}$, then 
    \begin{align*}
        \mathcal{E}_{test} \leq \epsilon
    \end{align*}
\end{proposition}

Training neural networks is basically a parameter estimation task. Thus, for a better understanding of PAC-theory, we begin with a trivial example, i.e., estimating the mean of bounded random variables. 
\begin{example}
     Let $X_1, \cdots, X_M$ be bounded i.i.d. random variables in $[b, b + B]$ and $y_i = g(x_i) = \mathbb{E}(X_i)$. 
\end{example}

We begin with the famous Hoeffding’s inequality. 
\begin{theorem} (Theorem 2.2.6 in \cite{vershynin2018high}) 
    Let $X_1, \cdots, X_M$ be bounded i.i.d. random variables in $[b, b + B]$. Then for any $t >0$, then exists an absolute constant $C$, such that 
    \begin{align*}
        \mathbb{P} \left\{ \sum_{i=1}^M \frac{1}{M} (X_i - \mathbb{E} X_i) \geq t \right\}  \leq \exp\left( -\frac{2t^2}{MB^2} \right).
    \end{align*}
\end{theorem}
Then we rewrite it in the terminology of PAC-learnable. 

\begin{proposition} (A Example of Learnability)\label{pro:high}
    Let $x_i$ be bounded random variables, $y_i = g(x_i) = \mathbb{E}(x_i)$, then $g$ is $(M, B\sqrt{\frac{1}{2M} \log \delta}, \delta)$-learnable and 
    \begin{align*}
        \mathcal{E}_{\text{test}} \leq B\sqrt{\frac{1}{2M} \log \delta}.
    \end{align*}
\end{proposition}

From Proposition \ref{pro:high}, the optimality gap is a decreasing function of sample complexity $M$.
